Half-turn symmetric FPLs with rare couplings and tilings of hexagons

In this work, we put to light a formula that relies the number of fully packed loop configurations (FPLs) associated to a given coupling pi to the number of half-turn symmetric FPLs (HTFPLs) of even size whose coupling is a punctured version of the coupling pi. When the coupling pi is the coupling with all arches parallel pi0 (the "rarest" one), this formula states the equality of the number of corresponding HTFPLs to the number of cyclically-symmetric plane partition of the same size. We provide a bijective proof of this fact. In the case of HTFPLs odd size, and although there is no similar expression, we study the number of HTFPLs whose coupling is a slit version of pi_0, and put to light new puzzling enumerative coincidence involving countings of tilings of hexagons and various symmetry classes of FPLs.

==> macros.tex <==
%% Macros pour dessins de glace carree

%% Fleches: a positionner au point de depart de la fleche
\newcommand{\flecheD}{\psline{->}(0,0)(.75,0)\psline(0,0)(1,0)}
\newcommand{\flecheG}{\psline{->}(0,0)(-.75,0)\psline(0,0)(-1,0)}
\newcommand{\flecheH}{\psline{->}(0,0)(0,.75)\psline(0,0)(0,1)}
\newcommand{\flecheB}{\psline{->}(0,0)(0,-.75)\psline(0,0)(0,-1)}

%% Grille carree: #1=nombre de lignes verticales #2=nombre de lignes horiz.
\newcounter{ISL}
\newcounter{ISH}
\newcommand{\IceGrid}[2]{%
\setcounter{ISL}{#1}\addtocounter{ISL}{-1}%
\setcounter{ISH}{#2}\addtocounter{ISH}{-1}%
\multido{\i=0+1}{#1}{\psline(\i,0)(\i,\theISH)}%
\multido{\i=0+1}{#2}{\psline(0,\i)(\theISL,\i)}%
}

%% Colonne de fleches vers la droite
\newcommand{\colD}[1]{%
\multido{\i=0+1}{#1}{\rput(0,\i){\flecheD}}%
}

%% Colonne de fleches vers la gauche
\newcommand{\colG}[1]{%
\multido{\i=0+1}{#1}{\rput(1,\i){\flecheG}}%
}

%% Ligne de fleches vers le haut
\newcommand{\linH}[1]{%
\multido{\i=0+1}{#1}{\rput(\i,0){\flecheH}}%
}

%% Ligne de fleches vers le bas
\newcommand{\linB}[1]{%
\multido{\i=0+1}{#1}{\rput(\i,1){\flecheB}}%
}

%% Colonne de traits horizontaux
\newcommand{\col}[1]{%
\multido{\i=0+1}{#1}{\rput(0,\i){\psline(0,0)(1,0)}}%
}

%% Ligne de traits verticaux
\newcommand{\lin}[1]{%
\multido{\i=0+1}{#1}{\rput(\i,0){\psline(0,0)(0,1)}}%
}

%% Serie de demi-cercles concentriques (x0,y0, rayon1, increment_reayon, nb)
%%% Pour une raison bizarre, il faut que le rayon et son increment aient
%%% le meme nombre de decimales
\newcommand{\halfCC}[5]{%
\degrees[360]%
\multido{\n=#3+#4}{#5}{\rput(#1,#2){\psarc(0,0){\n}{-90}{90}}}%
}

\newcommand{\tqCC}[5]{%
\degrees[360]%
\multido{\n=#3+#4}{#5}{\rput(#1,#2){\psarc(0,0){\n}{-90}{180}}}%
}

%% Glace carree classique
\newcommand{\IceSquare}[1]{%
\rput(1,1){\IceGrid{#1}{#1}}%
\rput(0,1){\colD{#1}}%
\rput(1,0){\linB{#1}}%
\rput(#1,1){\colG{#1}}%
\rput(1,#1){\linH{#1}}%
}

%% Glace carree ``HT'', paire, donner N/2 comme parametre
\newcounter{ISdoublesize}
\newcommand{\HTIceEven}[1]{%
\setcounter{ISdoublesize}{#1}\addtocounter{ISdoublesize}{#1}%
\rput(1,1){\IceGrid{#1}{\theISdoublesize}}%
\rput(0,1){\colD{\theISdoublesize}}%
\rput(1,0){\linB{#1}}%
\rput(1,\theISdoublesize){\linH{#1}}%
\rput(#1,#1){\rput(0,.5){\halfCC{0}{0}{.5}{1.0}{#1}}}%
\rput(#1,#1){\psline[linestyle=dotted](.25,.5)(.75,.5)}%
}

%% Glace carree ``HT'', impaire, donner (N-1)/2 comme parametre
\newcommand{\HTIceOdd}[1]{%
\setcounter{ISdoublesize}{#1}\addtocounter{ISdoublesize}{#1}%
\addtocounter{ISdoublesize}{1}%
\rput(1,1){\IceGrid{#1}{\theISdoublesize}}%
\rput(0,1){\colD{\theISdoublesize}}%
\rput(1,0){\linB{#1}}%
\rput(1,\theISdoublesize){\linH{#1}}%
\rput(#1,0){\psline(1,1)(1,#1)\rput(1,1){\flecheB}}%
\psarc(#1,#1){1}{0}{90}%
\rput(#1,#1){\halfCC{1}{1}{1}{1}{#1}}%
\rput(#1,1){\col{#1}}%
\rput(#1,#1){\rput(0,2){\col{#1}}}%
\rput(#1,#1){\psline[linestyle=dotted](.25,.25)(1.25,1.25)}%(#1,1)}%
%\rput(\theISdoublesize,#1){\psline[linestyle=dotted](.5,1)(-1,1)}%
}

%% Glace carree ``QT'', en vrai, parametre N/4
\newcounter{QTsize}
\newcommand{\QTIce}[1]{%
\setcounter{QTsize}{#1}\addtocounter{QTsize}{-1}%
\rput(1,1){\IceGrid{\theQTsize}{\theQTsize}}%
\rput(0,1){\colD{#1}}%
\rput(1,0){\linB{#1}}%
\rput(\theQTsize,1){\col{\theQTsize}}%
\rput(1,\theQTsize){\lin{\theQTsize}}%
\rput(\theQTsize,\theQTsize){\psarc(0,0){1}{0}{90}}%
\psline(1,#1)(\theQTsize,#1)\psline(#1,1)(#1,\theQTsize)%
\rput(#1,#1){\tqCC{0}{0}{1}{1}{\theQTsize}}%
\rput(#1,#1){\SpecialCoor\multido{\i=1+1}{\theQTsize}{\rput(\i;45){\psdots[dotstyle=*](0,0)}}}%
\rput(\theQTsize,\theQTsize){\SpecialCoor\psdots[dotstyle=*](1;45)\psline[linestyle=dotted](.5;45)(1.5;45)}%
}

%% Glace carree ``qQT'', parametre (N+2)/4
\newcommand{\qQTIce}[1]{%
\setcounter{QTsize}{#1}\addtocounter{QTsize}{-1}%
\rput(1,1){\IceGrid{\theQTsize}{\theQTsize}}%
\rput(0,1){\colD{#1}}%
\rput(1,0){\linB{#1}}%
\rput(\theQTsize,1){\col{\theQTsize}}%
\rput(1,\theQTsize){\lin{\theQTsize}}%
\rput(\theQTsize,\theQTsize){\psarc(0,0){1}{0}{90}}%
\psline(1,#1)(\theQTsize,#1)\psline(#1,1)(#1,\theQTsize)%
\rput(#1,#1){\tqCC{0}{0}{1}{1}{\theQTsize}}%
\rput(#1,#1){\SpecialCoor\multido{\i=1+1}{\theQTsize}{\rput(\i;45){\psdots[dotstyle=*](0,0)}}}%
\rput(\theQTsize,\theQTsize){\SpecialCoor\psline[linestyle=dotted](.5;45)(1.5;45)}%
}

%% Croisement dans un carre entre deux verticales
\newcommand{\Vcrossing}{%
\psbezier(0,0)(0,.4)(1,.6)(1,1)%
\psbezier(1,0)(1,.4)(0,.6)(0,1)%
}

%% Croisement dans un carre, entre deux horizontales
\newcommand{\Hcrossing}{%
\psbezier(0,0)(.4,0)(.6,1)(1,1)%
\psbezier(0,1)(.4,1)(.6,0)(1,0)%
}


%%% Zigouigouis pour indiquer des conditions au centre

\newcommand{\convcorner}{%
\begin{pspicture}(0.2,0.2)\psset{linewidth=.4pt,arrowsize=2.5pt}
\psline{->}(0,.2)(.2,.2)
\psline{->}(.2,0)(.2,.2)
\end{pspicture}%
}

\newcommand{\divcorner}{%
\begin{pspicture}(.2,.2)\psset{linewidth=.4pt,arrowsize=2.5pt}
\psline{->}(.2,.2)(.2,0)
\psline{->}(.2,.2)(0,.2)
\end{pspicture}%
}

\newcommand{\upleft}{%
\begin{pspicture}(.2,.2)\psset{linewidth=.4pt,arrowsize=2.5pt}
\psline(.2,0)(.2,.15)\psarc(.15,.15){.05}{0}{90}\psline{->}(.15,.2)(0,.2)%
\end{pspicture}%
}

\newcommand{\downright}{%
\begin{pspicture}(.2,.2)\psset{linewidth=.4pt,arrowsize=2.5pt}
\psline(0,.2)(.15,.2)\psarc(.15,.15){.05}{0}{90}\psline{->}(.2,.15)(.2,0)%
\end{pspicture}
}

\newcommand{\upc}{%
\begin{pspicture}(.2,.2)\psset{linewidth=.4pt,arrowsize=2.5pt}%
\psline(0,0)(.1,0)\psarc(.1,.1){.1}{270}{90}\psline{->}(.1,.2)(0,.2)%
\end{pspicture}%
}

\newcommand{\downc}{%
\begin{pspicture}(.2,.2)\psset{linewidth=.4pt,arrowsize=2.5pt}%
\psline(0,.2)(.1,.2)\psarc(.1,.1){.1}{270}{90}\psline{->}(.1,0)(0,0)%
\end{pspicture}%
}

\newcommand{\ZqConv}{%
Z_{\textsc{QT}}^{\convcorner}%
}

\newcommand{\ZqDiv}{%
Z_{\textsc{QT}}^{\divcorner}%
}

\newcommand{\ZqUpleft}{%
Z_{\textsc{QT}}^{\upleft}%
}

\newcommand{\ZqDownright}{%
Z_{\textsc{QT}}^{\downright}%
}

\newcommand{\ZhUp}{%
Z_{\textsc{HT}}^{\upc}%
}

\newcommand{\ZhDown}{%
Z_{\textsc{HT}}^{\downc}%
}


\newcommand{\ZhUpleft}{%
Z_{\textsc{HT}}^{\upleft}%
}

\newcommand{\ZhDownright}{%
Z_{\textsc{HT}}^{\downright}%
}

\newrgbcolor{lightblue}{.5 .5 1}
\newrgbcolor{lightpink}{1 .5 .5}

\newcommand{\CarreB}{%
\psframe*[linecolor=lightblue](.15,.15)(.85,.85)%
}

\newcommand{\DominoHB}{%
\psframe*[linecolor=lightblue](.15,.15)(1.85,.85)%
}

\newcommand{\DominoVB}{%
\psframe*[linecolor=lightblue](.15,.15)(.85,1.85)%
}

\newcommand{\CarreR}{%
\psframe*[linecolor=lightpink](.15,.15)(.85,.85)%
}

\newcommand{\DominoHR}{%
\psframe*[linecolor=lightpink](.15,.15)(1.85,.85)%
}

\newcommand{\DominoVR}{%
\psframe*[linecolor=lightpink](.15,.15)(.85,1.85)%
}


